Audio-Visual Speech Codecs: Rethinking Audio-Visual Speech Enhancement by Re-Synthesis

Since facial actions such as lip movements contain significant information about speech content, it is not surprising that audio-visual speech enhancement methods are more accurate than their audio-only counterparts. Yet, state-of-the-art approaches still struggle to generate clean, realistic speech without noise artifacts and unnatural distortions in challenging acoustic environments. In this paper, we propose a novel audio-visual speech enhancement framework for high-fidelity telecommunications in AR/VR. Our approach leverages audio-visual speech cues to generate the codes of a neural speech codec, enabling efficient synthesis of clean, realistic speech from noisy signals. Given the importance of speaker-specific cues in speech, we focus on developing personalized models that work well for individual speakers. We demonstrate the efficacy of our approach on a new audio-visual speech dataset collected in an unconstrained, large vocabulary setting, as well as existing audio-visual datasets, outperforming speech enhancement baselines on both quantitative metrics and human evaluation studies. Please see the supplemental video for qualitative results at https://github.com/facebookresearch/facestar/releases/download/paper_materials/video.mp4.

==> subfiles/old/experiments.tex <==
\section{Experiments}
We train and evaluate our single-speaker model on five speakers from the new Facestar dataset (described below) and five speakers from the YouTube-Lip2Wav dataset \cite{prajwal2020learning}.



















\iffalse

\begin{table*}[]
\footnotesize
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{Noise   Type} & \textbf{Model} & \textbf{PESQ}  & \textbf{STOI}  & \textbf{SRMR}  & \textbf{FW-SSNR} & \textbf{MCD}   & \textbf{CSIG}  & \textbf{CBAK}  & \textbf{COVL}  & \textbf{Mel-Spec-Dist} \\ \hline
VCTK + Audioset       & AV Baseline    & 1.333          & 0.624          & 8.083          & 6.44             & 4.86           & 2.656          & 1.803          & 1.919          & 0.008                  \\ \hline
VCTK + Audioset       & Ours           & 1.412          & 0.664          & 8.47           & 7.593            & 3.437          & 3.101          & 1.849          & 2.2            & 0.004                  \\ \hline
VCTK + Audioset       & Ours + AR      & \textbf{1.461} & \textbf{0.682} & \textbf{8.94}  & \textbf{7.811}   & \textbf{3.258} & \textbf{3.196} & \textbf{1.893} & \textbf{2.279} & \textbf{0.004}         \\ \hline
VoxCeleb2 + Audioset  & AV Baseline    & 1.234          & 0.567          & 6.744          & 5.51             & 4.99           & 2.472          & 1.71           & 1.752          & 0.009                  \\ \hline
VoxCeleb2 + Audioset  & Ours           & 1.278          & 0.608          & 8.314          & 6.765            & 3.758          & 2.877          & 1.754          & 2.007          & 0.005                  \\ \hline
VoxCeleb2 + Audioset  & Ours + AR      & \textbf{1.384} & \textbf{0.651} & \textbf{9.184} & \textbf{7.409}   & \textbf{3.453} & \textbf{3.079} & \textbf{1.837} & \textbf{2.177} & \textbf{0.005}         \\ \hline
\end{tabular}
\caption{Facestar results}
\label{table:facestarj}
\end{table*}



\begin{table*}[]
\scriptsize
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{Dataset} & \textbf{Noise   Type}     & \textbf{Model} & \textbf{PESQ}                & \textbf{STOI}  & \textbf{SRMR}  & \textbf{FW-SSNR} & \textbf{MCD}   & \textbf{CSIG}  & \textbf{CBAK}  & \textbf{COVL}  & \textbf{Mel-Spec-Dist} \\ \hline
Eh               & VoxCeleb2 + Audioset + IR & AV Baseline    & 1.38733 / 1.86672            & 0.655          & 9.407          & 7.539            & 4.888          & 2.7            & 1.651          & 1.955          & 0.008                  \\ \hline
Eh               & VoxCeleb2 + Audioset + IR & Ours           & \textbf{1.40612 / 1.85986}   & \textbf{0.693} & \textbf{13.53} & \textbf{8.347}   & \textbf{3.726} & \textbf{2.956} & \textbf{1.781} & \textbf{2.102} & \textbf{0.005}         \\ \hline
Hs               & VoxCeleb2 + Audioset + IR & AV Baseline    & \textbf{1.52059 / 1.92807}   & \textbf{0.664} & 11.04          & 7.412            & 5.18           & 2.699          & \textbf{1.701} & \textbf{2.022} & 0.01                   \\ \hline
Hs               & VoxCeleb2 + Audioset + IR & Ours           & 1.42169 / 1.75007            & 0.658          & \textbf{12.51} & \textbf{7.427}   & \textbf{4.6}   & \textbf{2.749} & 1.655          & 1.995          & \textbf{0.008}         \\ \hline
Dl               & VoxCeleb2 + Audioset + IR & AV Baseline    & \textbf{1.53896 / 1.93040}   & 0.651          & 9.759          & 8.101            & 5.099          & 2.758          & 1.728          & 2.069          & 0.01                   \\ \hline
Dl               & VoxCeleb2 + Audioset + IR & Ours           & 1.50872 / 1.82999            & \textbf{0.69}  & \textbf{11.77} & \textbf{8.466}   & \textbf{4.294} & \textbf{2.899} & \textbf{1.776} & \textbf{2.125} & \textbf{0.006}         \\ \hline
Chess            & VoxCeleb2 + Audioset + IR & AV Baseline    & \textbf{1.42596   / 1.92076} & 0.756          & \textbf{4.056} & 9.128            & 5.069          & 2.868          & 1.833          & 2.113          & 0.007                  \\ \hline
Chess            & VoxCeleb2 + Audioset + IR & Ours           & 1.37996 / 1.82081            & \textbf{0.776} & 3.075          & \textbf{9.56}    & \textbf{4.313} & \textbf{3.001} & \textbf{1.841} & \textbf{2.153} & \textbf{0.005}         \\ \hline
Chem             & VoxCeleb2 + Audioset + IR & AV Baseline    & 1.31894 / 1.70456            & 0.717          & 7.107          & 7.187            & 5.598          & 2.476          & 1.591          & 1.81           & 0.012                  \\ \hline
Chem             & VoxCeleb2 + Audioset + IR & Ours           & \textbf{1.48055 / 1.92168}   & \textbf{0.798} & \textbf{10.14} & \textbf{8.966}   & \textbf{3.882} & \textbf{3.053} & \textbf{1.853} & \textbf{2.207} & \textbf{0.006}         \\ \hline
\end{tabular}
\caption{YouTube-Lip2Wav Results}
\label{table:lip2wav}
\end{table*}

\fi
